Fast Algorithms for Knapsack via Convolution and Prediction

The \Problem{knapsack} problem is a fundamental problem in combinatorial optimization. It has been studied extensively from theoretical as well as practical perspectives as it is one of the most well-known NP-hard problems. The goal is to pack a knapsack of size $t$ with the maximum value from a collection of $n$ items with given sizes and values. Recent evidence suggests that a classic $O(nt)$ dynamic-programming solution for the \Problem{knapsack} problem might be the fastest in the worst case. In fact, solving the \Problem{knapsack} problem was shown to be computationally equivalent to the \Problem{$(\min, +)$ convolution} problem, which is thought to be facing a quadratic-time barrier. This hardness is in contrast to the more famous \Problem{$(+, \cdot)$ convolution} (generally known as \Problem{polynomial multiplication}), that has an $O(n\log n)$-time solution via Fast Fourier Transform. Our main results are algorithms with near-linear running times (in terms of the size of the knapsack and the number of items) for the \Problem{knapsack} problem, if either the values or sizes of items are small integers. More specifically, if item sizes are integers bounded by $\smax$, the running time of our algorithm is $\tilde O((n+t)\smax)$. If the item values are integers bounded by $\vmax$, our algorithm runs in time $\tilde O(n+t\vmax)$. Best previously known running times were $O(nt)$, $O(n^2\smax)$ and $O(n\smax\vmax)$ (Pisinger, J. of Alg., 1999).

==> figs/windows.tex <==
\begin{figure}[h!]

\begin{center}
\begin{tikzpicture}[scale=0.96, transform shape]

%\draw (0,0) -- (15.4,0) -- (15.4,0.5) -- (0,0.5) -- (0,0);
%\node[text width=3cm] at (9,0.2) 
%{$a$};

%\node[text width=3cm, rotate = 90] at (-0.5,2.6) 
%{    \Huge$\overbrace{\hspace{3.9cm}}$   };
%\node[text width=3cm, rotate = 90] at (-1.3,3.2) 
%{  $\log n +1$ rounds  };

%\node[text width=3cm] at (3.9,5.2) 
%{    \huge$\overbrace{\hspace{3.0cm}}$   };



\node[text width=3cm, rotate = 90] at (7.72,4.1) 
{  \huge  $\ldots$   };

\draw (-0.1,1.1) -- (15.5,1.1) -- (15.5,1.8) -- (-0.1,1.8) -- (-0.1,1.1);
\draw[dashed] (0,1.2) -- (0.4,1.2) -- (0.4,1.7) -- (0,1.7) -- (0,1.2);
\draw[dashed] (0.5,1.2) -- (0.9,1.2) -- (0.9,1.7) -- (0.5,1.7) -- (0.5,1.2);
\draw[dashed] (1,1.2) -- (1.4,1.2) -- (1.4,1.7) -- (1,1.7) -- (1,1.2);
\draw[dashed] (1.5,1.2) -- (1.9,1.2) -- (1.9,1.7) -- (1.5,1.7) -- (1.5,1.2);
\draw[dashed] (2,1.2) -- (2.4,1.2) -- (2.4,1.7) -- (2,1.7) -- (2,1.2);
\draw[dashed] (2.5,1.2) -- (2.9,1.2) -- (2.9,1.7) -- (2.5,1.7) -- (2.5,1.2);
\draw[dashed] (3,1.2) -- (3.4,1.2) -- (3.4,1.7) -- (3,1.7) -- (3,1.2);
\draw[dashed] (3.5,1.2) -- (3.9,1.2) -- (3.9,1.7) -- (3.5,1.7) -- (3.5,1.2);
\draw[dashed] (4,1.2) -- (4.4,1.2) -- (4.4,1.7) -- (4,1.7) -- (4,1.2);
\draw[dashed] (4.5,1.2) -- (4.9,1.2) -- (4.9,1.7) -- (4.5,1.7) -- (4.5,1.2);
\draw[dashed] (5,1.2) -- (5.4,1.2) -- (5.4,1.7) -- (5,1.7) -- (5,1.2);
\draw[dashed] (5.5,1.2) -- (5.9,1.2) -- (5.9,1.7) -- (5.5,1.7) -- (5.5,1.2);
\draw[dashed] (6,1.2) -- (6.4,1.2) -- (6.4,1.7) -- (6,1.7) -- (6,1.2);
\draw[dashed] (6.5,1.2) -- (6.9,1.2) -- (6.9,1.7) -- (6.5,1.7) -- (6.5,1.2);



\draw[dashed] (8.5,1.2) -- (8.9,1.2) -- (8.9,1.7) -- (8.5,1.7) -- (8.5,1.2);
\draw[dashed] (9,1.2) -- (9.4,1.2) -- (9.4,1.7) -- (9,1.7) -- (9,1.2);
\draw[dashed] (9.5,1.2) -- (9.9,1.2) -- (9.9,1.7) -- (9.5,1.7) -- (9.5,1.2);
\draw[dashed] (10,1.2) -- (10.4,1.2) -- (10.4,1.7) -- (10,1.7) -- (10,1.2);
\draw[dashed] (10.5,1.2) -- (10.9,1.2) -- (10.9,1.7) -- (10.5,1.7) -- (10.5,1.2);
\draw[dashed] (11,1.2) -- (11.4,1.2) -- (11.4,1.7) -- (11,1.7) -- (11,1.2);
\draw[dashed] (11.5,1.2) -- (11.9,1.2) -- (11.9,1.7) -- (11.5,1.7) -- (11.5,1.2);
\draw[dashed] (12,1.2) -- (12.4,1.2) -- (12.4,1.7) -- (12,1.7) -- (12,1.2);
\draw[dashed] (12.5,1.2) -- (12.9,1.2) -- (12.9,1.7) -- (12.5,1.7) -- (12.5,1.2);
\draw[dashed] (13,1.2) -- (13.4,1.2) -- (13.4,1.7) -- (13,1.7) -- (13,1.2);
\draw[dashed] (13.5,1.2) -- (13.9,1.2) -- (13.9,1.7) -- (13.5,1.7) -- (13.5,1.2);
\draw[dashed] (14,1.2) -- (14.4,1.2) -- (14.4,1.7) -- (14,1.7) -- (14,1.2);
\draw[dashed] (14.5,1.2) -- (14.9,1.2) -- (14.9,1.7) -- (14.5,1.7) -- (14.5,1.2);
\draw[dashed] (15,1.2) -- (15.4,1.2) -- (15.4,1.7) -- (15,1.7) -- (15,1.2);
%\draw[dashed] (6.2,1.2) -- (9.2,1.2) -- (9.2,1.7) -- (6.2,1.7) -- (6.2,1.2);
\node[text width=3cm] at (8.8,1.4) 
{   \huge $\ldots$   };

\node[text width=3cm] at (17.1,1.4) 
{   round $\log n +1$  };

%\draw[dashed] (9.3,1.2) -- (12.3,1.2) -- (12.3,1.7) -- (9.3,1.7) -- (9.3,1.2);
%\draw[dashed] (12.4,1.2) -- (15.4,1.2) -- (15.4,1.7) -- (12.4,1.7) -- (12.4,1.2);

%\draw[dashed] (0.6,2) -- (3.6,2) -- (3.6,2.5) -- (0.6,2.5) -- (0.6,2);
%\draw[dashed] (3.7,2) -- (6.7,2) -- (6.7,2.5) -- (3.7,2.5) -- (3.7,2);
%\draw[dashed] (6.8,2) -- (9.8,2) -- (9.8,2.5) -- (6.8,2.5) -- (6.8,2);

\draw (-0.1,1.9) -- (15.5,1.9) -- (15.5,2.6) -- (-0.1,2.6) -- (-0.1,1.9);
\draw[dashed] (0,2) -- (0.9,2) -- (0.9,2.5) -- (0,2.5) -- (0,2);
\draw[dashed] (1,2) -- (1.9,2) -- (1.9,2.5) -- (1,2.5) -- (1,2);
\draw[dashed] (2,2) -- (2.9,2) -- (2.9,2.5) -- (2,2.5) -- (2,2);
\draw[dashed] (3,2) -- (3.9,2) -- (3.9,2.5) -- (3,2.5) -- (3,2);
\draw[dashed] (4,2) -- (4.9,2) -- (4.9,2.5) -- (4,2.5) -- (4,2);
\draw[dashed] (5,2) -- (5.9,2) -- (5.9,2.5) -- (5,2.5) -- (5,2);
\draw[dashed] (6,2) -- (6.9,2) -- (6.9,2.5) -- (6,2.5) -- (6,2);


\draw[dashed] (8.5,2) -- (9.4,2) -- (9.4,2.5) -- (8.5,2.5) -- (8.5,2);
\draw[dashed] (9.5,2) -- (10.4,2) -- (10.4,2.5) -- (9.5,2.5) -- (9.5,2);
\draw[dashed] (10.5,2) -- (11.4,2) -- (11.4,2.5) -- (10.5,2.5) -- (10.5,2);
\draw[dashed] (11.5,2) -- (12.4,2) -- (12.4,2.5) -- (11.5,2.5) -- (11.5,2);
\draw[dashed] (12.5,2) -- (13.4,2) -- (13.4,2.5) -- (12.5,2.5) -- (12.5,2);
\draw[dashed] (13.5,2) -- (14.4,2) -- (14.4,2.5) -- (13.5,2.5) -- (13.5,2);
\draw[dashed] (14.5,2) -- (15.4,2) -- (15.4,2.5) -- (14.5,2.5) -- (14.5,2);

\node[text width=3cm] at (8.8,2.2) 
{   \huge $\ldots$   };
%\draw[dashed] (9.9,2) -- (12.9,2) -- (12.9,2.5) -- (9.9,2.5) -- (9.9,2);
\node[text width=3cm] at (17.1,2.2) 
{   round $\log n$  };


%\draw[dashed] (1.2,2.8) -- (4.2,2.8) -- (4.2,3.3) -- (1.2,3.3) -- (1.2,2.8);
%\draw[dashed] (4.3,2.8) -- (7.3,2.8) -- (7.3,3.3) -- (4.3,3.3) -- (4.3,2.8);
%\draw[dashed] (7.4,2.8) -- (10.4,2.8) -- (10.4,3.3) -- (7.4,3.3) -- (7.4,2.8);
%\node[text width=3cm] at (10.0,3.0) 
%{   \huge $\ldots$   };
%\draw[dashed] (10.5,2.8) -- (13.5,2.8) -- (13.5,3.3) -- (10.5,3.3) -- (10.5,2.8);

\draw (-0.1,3.5) -- (15.5,3.5) -- (15.5,4.2) -- (-0.1,4.2) -- (-0.1,3.5);
\draw[dashed] (0,3.6) -- (7.6,3.6) -- (7.6,4.1) -- (0,4.1) -- (0,3.6);
%\draw[dashed] (1.8,3.6) -- (4.8,3.6) -- (4.8,4.1) -- (1.8,4.1) -- (1.8,3.6);
%\draw[dashed] (4.9,3.6) -- (7.9,3.6) -- (7.9,4.1) -- (4.9,4.1) -- (4.9,3.6);
%\draw[dashed] (8.0,3.6) -- (11.0,3.6) -- (11.0,4.1) -- (8.0,4.1) -- (8.0,3.6);
\draw[dashed] (7.8,3.6) -- (15.4,3.6) -- (15.4,4.1) -- (7.8,4.1) -- (7.8,3.6);
%\draw[dashed] (11.1,3.6) -- (14.1,3.6) -- (14.1,4.1) -- (11.1,4.1) -- (11.1,3.6);

\node[text width=3cm] at (17.1,3.8) 
{   round $2$  };

\draw (-0.1,4.3) -- (15.5,4.3) -- (15.5,5) -- (-0.1,5) -- (-0.1,4.3);
\draw[dashed] (0,4.4) -- (15.4,4.4) -- (15.4,4.9) -- (0,4.9) -- (0,4.4);
\node[text width=3cm] at (17.1,4.6) 
{   round $1$  };

\node[text width=3cm] at (1.42,5.3) 
{   $1$   };
\node[text width=3cm] at (16.62,5.3) 
{   $n$   };
%\draw[dashed] (2.4,4.4) -- (5.4,4.4) -- (5.4,4.9) -- (2.4,4.9) -- (2.4,4.4);
%\draw[dashed] (5.5,4.4) -- (8.5,4.4) -- (8.5,4.9) -- (5.5,4.9) -- (5.5,4.4);
%\draw[dashed] (8.6,4.4) -- (11.6,4.4) -- (11.6,4.9) -- (8.6,4.9) -- (8.6,4.4);
%\node[text width=3cm] at (11.2,4.6) 
%{   \huge $\ldots$   };
%\draw[dashed] (11.7,4.4) -- (14.7,4.4) -- (14.7,4.9) -- (11.7,4.9) -- (11.7,4.4);




%\node [draw,rounded corners,minimum height=5cm,minimum width=4cm] (node1) {};
%\node [anchor=north west,minimum width=10cm] at (-3.6,1) {\fbox{\hspace{1cm}$w_1$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (-0.9,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (1.8,1) {\fbox{\hspace{1cm}$\ldots$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (4.5,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (7.2,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (0,0) {\fbox{\hspace{6.4cm}$s_1$\hspace{6.4cm}}};
% {\fbox{\hspace{6.4cm}$s_1$\hspace{6.4cm}}};

%\node [anchor=south west] at (node1.north west) {\fbox{Case: anchor is SW}};
%\node [anchor=south east] at (node1.north west) {\fbox{Case: anchor is SE}};
%\node [anchor=north east] at (node1.north west) {\fbox{Case: anchor is NE}};
%\foreach \myanchor in {north west}
%{ 
%	\node[fill,circle,inner sep=1pt,outer sep=1ex,anchor=\myanchor] at (node1.north west){};
%}
\end{tikzpicture}
\end{center}
\caption{In every round $s+1$, $b$ is split into $2^s$ intervals of size $2^{\log n - s}$.}\label{figs:bs}
\end{figure}

==> path1.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[
% Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,
		anchor=east,xshift=-1mm},
    be/.style={circle,thick,draw,fill=green!60,anchor=north,
		minimum width=0.7cm},
    tr/.style={buffer gate US,thick,draw,fill=purple!60,rotate=90,
		anchor=east,minimum width=0.8cm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=7cm,level distance=1.4cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=7cm},
    level 3/.style={sibling distance=6cm},
    level 4/.style={sibling distance=3cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
 %% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node. 

%% Draw system flow diagram
   \begin{scope}[xshift=-7.5cm,yshift=-5cm,very thick,
		node distance=1.6cm,on grid,>=stealth',
		block/.style={rectangle,draw,fill=cyan!20},
		comp/.style={thin,rectangle,draw,fill=white!40}]
   \node [block] (re)					{bounded tree sparsity};
    \node[comp] (re')[below=of re, yshift=0.5cm] {$\tildorder(\wmax n)$};
   \node [block] (re2)				[right= of re, xshift=3cm]	{bounded tree separability};
    \node[comp] (re'2)[below=of re2, yshift=0.5cm] {$\tildorder(\wmax n)$};
   \node [block] (re3)				[right= of re2, xshift=3cm]	{bounded knapsack};
    \node[comp] (re'3)[below=of re3, yshift=0.5cm] {$\tildorder(\vmax n)$};
   \node [block] (re4)				[right= of re3, xshift=3cm]	{bounded convolution};
   \node[comp] (re'4)[below=of re4, yshift=0.5cm] {$\tildorder(\emax n)$};
   \node [block]	 (ca1)	[above=of re2,xshift=1.8cm]	{$\dmax$-distance bounded convolution} edge [->] (re) edge [->] (re2) edge [->] (re3) edge [->] (re4);
   \node[comp] (ca'1)[right=of ca1, xshift=3cm] {$\tildorder(\dmax n)$};
   \node [block] (s1)	[above=of ca1]		{$0/1$ tree sparsity} edge [->] (ca1);
   \node[comp] (s'1)[right=of s1, xshift=1cm] {$\tildorder(n)$};
   \draw[very thick,->]  (re.north west) -- (s1.west);
   \draw[dotted,thin] (s1) -- (s'1);
   \draw[dotted,thin] (ca1) -- (ca'1);
    \draw[dotted,thin] (re) -- (re');
        \draw[dotted,thin] (re2) -- (re'2);
            \draw[dotted,thin] (re3) -- (re'3);
                \draw[dotted,thin] (re4) -- (re'4);
   \end{scope}
\end{tikzpicture}
\caption{Desired running times are specified in the white boxes. $a \rightarrow b$ means an efficient algorithm for $a$ yields an efficient algorithm for $b$.}\label{fig:reductions}
\end{figure}

==> path2.tex <==
\tikzstyle{H-node}=[rectangle,draw=black,fill=white!30,inner sep=1.3mm]
\tikzstyle{B-node}=[circle,draw=blue,fill=blue!20,inner sep=2.5mm]
\tikzstyle{G-node}=[circle,draw=black,fill=white!30,inner sep=3.3mm]
\tikzstyle{R-node}=[rectangle,draw=red,fill=red!20,inner sep=2.6mm]
\tikzstyle{W-node}=[rectangle,draw=white,fill=white!30,inner sep=0.2mm]
\tikzstyle{test-node}=[circle,draw=black,fill=black,inner sep=.2mm]

\tikzstyle{bl0} = [draw=black, thick, dashed]   
\tikzstyle{b9} = [draw=red, thick]   
\tikzstyle{b8} = [draw=blue, thick, dotted]   
\tikzstyle{bl1} = [->, draw=black]   
\tikzstyle{bl2} = [draw=black!70,thick]   
\tikzstyle{bl3} = [draw=black,thick, dotted]   

\tikzstyle{br0} = [draw=brown, dashed]   
\tikzstyle{br1} = [->, draw=brown]   
\tikzstyle{br2} = [->, draw=brown,thick]   

\tikzstyle{red0} = [draw=red, thick, dashed]   
\tikzstyle{red1} = [draw=red]   
\tikzstyle{red2} = [draw=red,thick]   

\tikzstyle{gr0} = [draw=green, thick, dashed]   
\tikzstyle{gr1} = [draw=green]   
\tikzstyle{gr2} = [draw=green,thick]   
\tikzstyle{gr4} = [draw=green,semithick,rounded corners]   

\begin{figure}%[!htbp]
\begin{center}
\begin{tikzpicture}[scale=0.5][domain=0:8]%,dash pattern=on 2pt off 3pt on 4pt off 4pt]
\draw (0,0) node[G-node,label=center:$r$,label=below:] (r) {};
\draw (0,3) node[G-node,label=center:$c'_{0}$,label=below:] (c'_0) {};
\draw (0,6) node[G-node,label=center:$c'_{1}$,label=below:] (c'_1) {};
\draw (0,9) node[G-node,label=center:$c'_{2}$,label=below:] (c'_2) {};
\draw (0,13) node[G-node,label=center:$c'_{2n-2}$,label=below:$\vdots$] (c'_{2n-2}) {};

\draw (-3,0) node[G-node,label=center:$a'_{0}$,label=below:] (a'_0) {};
\draw (-6,0) node[G-node,label=center:$a'_{1}$,label=below:] (a'_1) {};
\draw (-9.3,0) node[G-node,label=center:$a'_{n-1}$,label=right:$\ldots$] (a'_{n-1}) {};
\draw (-12.3,0) node[G-node,label=center:$a'_{n}$,label=below:] (a'_{n}) {};
\draw (-15.6,0) node[G-node,label=center:$a'_{2n-1}$,label=right:$\ldots$] (a'_{2n-1}) {};
\draw (-15.6,3) node[G-node,label=center:$a'_{2n}$] (a'_{2n}) {};
\draw (-15.6,6) node[G-node,label=center:$a'_{2n+1}$] (a'_{2n+1}) {};
\draw (-15.6,9) node[G-node,label=center:$a'_{2n+2}$] (a'_{2n+2}) {};
\draw (-15.6,13) node[G-node,label=center:$a'_{3n-1}$,label=below:$\vdots$] (a'_{3n-1}) {};



\draw (3,0) node[G-node,label=center:$b'_{0}$,label=below:] (b'_0) {};
\draw (6,0) node[G-node,label=center:$b'_{1}$,label=below:] (b'_1) {};
\draw (9.3,0) node[G-node,label=center:$b'_{n-1}$,label=left:$\ldots$] (b'_{n-1}) {};
\draw (12.3,0) node[G-node,label=center:$b'_{n}$,label=below:] (b'_{n}) {};
\draw (15.6,0) node[G-node,label=center:$b'_{2n-1}$,label=left:$\ldots$] (b'_{2n-1}) {};
\draw (15.6,3) node[G-node,label=center:$b'_{2n}$] (b'_{2n}) {};
\draw (15.6,6) node[G-node,label=center:$b'_{2n+1}$] (b'_{2n+1}) {};
\draw (15.6,9) node[G-node,label=center:$b'_{2n+2}$] (b'_{2n+2}) {};
\draw (15.6,13) node[G-node,label=center:$b'_{3n-1}$,label=below:$\vdots$] (b'_{3n-1}) {};

\draw[b9] (r)  to node [below,label=right:$M+c_{2n-2}$] {} (c'_0) ;
\draw[b9] (c'_0)  to node [below,label=right:$M+c_{2n-3}$] {} (c'_1) ;
\draw[b9] (c'_1)  to node [below,label=right:$M+c_{2n-4}$] {} (c'_2) ;
\draw[b8] (r)  to node [below,label=below:$\infty$] {} (a'_0) ;
\draw[b8] (a'_0)  to node [below,label=below:$\infty$] {} (a'_1) ;
\draw[b9] (a'_{n-1})  to node [below,label=below:$M-a_0$] {} (a'_{n}) ;
\draw[b8] (a'_{2n-1})  to node [below,label=right:$\infty$] {} (a'_{2n}) ;
\draw[b8] (a'_{2n})  to node [below,label=right:$\infty$] {} (a'_{2n+1}) ;
\draw[b8] (a'_{2n+1})  to node [below,label=right:$\infty$] {} (a'_{2n+2}) ;

\draw[b8] (b'_{2n-1})  to node [below,label=left:$\infty$] {} (b'_{2n}) ;
\draw[b8] (b'_{2n})  to node [below,label=left:$\infty$] {} (b'_{2n+1}) ;
\draw[b8] (b'_{2n+1})  to node [below,label=left:$\infty$] {} (b'_{2n+2}) ;


\draw[b8] (r)  to node [below,label=below:$\infty$] {} (b'_0) ;
\draw[b8] (b'_0)  to node [below,label=below:$\infty$] {} (b'_1) ;
\draw[b9] (b'_{n-1})  to node [below,label=below:$M-b_0$] {} (b'_{n}) ;

%\draw[b9] (b_2)  to node [label=right:$q_{B1}$] {} (h_1) ;
%\draw (3, 8) node[W-node,label=center:First Scenario] (s1) {};

%\draw (9,5) node[B-node,label=center:$A$,label=below:$\pi_A$\text{$=$}$0.0938$] (bb_1) {};
%\draw (13,5) node[B-node,label=center:$B$,label=below:$\pi_B$\text{$=$}$0.0938$] (bb_2) {};
%\draw (9,0) node[R-node,label=center:$1$, label=below:$p_1$\text{$=$}$\frac{1}{2}$] (hh_1) {};
%\draw (13,0) node[R-node,label=center:$2$, label=below:$p_2$\text{$=$}$\frac{1}{2}$] (hh_2) {};

%\draw[b9] (bb_1) to node [label=left:$q_{A1}$] {} (hh_1) ;
%\draw[b9] (bb_1) -- (hh_2) ;
%\draw[b9] (bb_2) -- (hh_1) ;
%\draw[b9] (bb_2) to node [label=right:$q_{B2}$] {} (hh_2) ;
%\draw (11, 8) node[W-node,label=center:Second Scenario] (s2) {};

%\draw (9.8, 3) node[W-node,label=center:$q_{A2}$] (lab2) {};
%\draw (12.2, 3) node[W-node,label=center:$q_{B1}$] (lab3) {};

%\draw (17,5) node[B-node,label=center:$A$,label=below:$\pi_A$\text{$=$}$0.124$] (bbb_1) {};
%\draw (21,5) node[B-node,label=center:$B$,label=below:$\pi_B$\text{$=$}$0.064$] (bbb_2) {};
%\draw (17,0) node[R-node,label=center:$1$, label=below:$p_1$\text{$=$}$0.64$] (hhh_1) {};
%\draw (21,0) node[R-node,label=center:$2$, label=below:$p_2$\text{$=$}$0.48$] (hhh_2) {};

%\draw[b9] (bbb_1)  to node [label=left:$q_{A1}$] {} (hhh_1) ;
%\draw[b9] (bbb_1)  to node [label=left:$q_{A2}$] {} (hhh_2) ;
%\draw[b9] (bbb_2)  to node [label=right:$q_{B2}$] {} (hhh_2) ;
%\draw (19, 8) node[W-node,label=center:Third Scenario] (s3) {};
\end{tikzpicture}
\end{center}
\caption{Dashed edges have weight $\infty$ while the weight of the solid edges is based on the value of the vectors $a$, $b$, and $c$.}
\label{fig:treeseparability}
\end{figure}

==> path3.tex <==
\tikzstyle{H-node}=[rectangle,draw=black,fill=white!30,inner sep=1.3mm]
\tikzstyle{B-node}=[circle,draw=blue,fill=blue!20,inner sep=2.5mm]
\tikzstyle{G-node}=[circle,draw=black,fill=white!30,inner sep=3.3mm]
\tikzstyle{R-node}=[rectangle,draw=red,fill=red!20,inner sep=2.6mm]
\tikzstyle{W-node}=[rectangle,draw=white,fill=white!30,inner sep=0.2mm]
\tikzstyle{test-node}=[circle,draw=black,fill=black,inner sep=.2mm]

\tikzstyle{bl0} = [draw=black, thick, dashed]   
\tikzstyle{b9} = [draw=red, thick]   
\tikzstyle{b8} = [draw=blue, thick, dotted]   
\tikzstyle{bl1} = [->, draw=black]   
\tikzstyle{bl2} = [draw=black!70,thick]   
\tikzstyle{bl3} = [draw=black,thick, dotted]   

\tikzstyle{br0} = [draw=brown, dashed]   
\tikzstyle{br1} = [->, draw=brown]   
\tikzstyle{br2} = [->, draw=brown,thick]   

\tikzstyle{red0} = [draw=red, thick, dashed]   
\tikzstyle{red1} = [draw=red]   
\tikzstyle{red2} = [draw=red,thick]   

\tikzstyle{gr0} = [draw=green, thick, dashed]   
\tikzstyle{gr1} = [draw=green]   
\tikzstyle{gr2} = [draw=green,thick]   
\tikzstyle{gr4} = [draw=green,semithick,rounded corners]   

\begin{figure}%[!htbp]
\begin{center}
\begin{tikzpicture}[scale=0.5][domain=0:8]%,dash pattern=on 2pt off 3pt on 4pt off 4pt]
\draw (0,0) node[G-node,label=center:$1$,label=below:,label=below:$r$] (r) {};
\draw (0,3) node[G-node,label=center:$1$,label=below:,label=right:$c'_1$] (c'_1) {};
\draw (0,6) node[G-node,label=center:$1$,label=below:,label=right:$c'_2$] (c'_2) {};
\draw (0,10) node[G-node,label=center:$1$,label=below:$\vdots$,label=right:$c'_8$] (c'_8) {};
\draw (0,13) node[G-node,label=center:$1$,label=right:$c'_9$] (c'_9) {};

\draw (-3,0) node[G-node,label=center:$1$,label=below:$a'_1$] (a'_1) {};
\draw (-6,0) node[G-node,label=center:$0$,label=below:$a'_2$] (a'_2) {};
\draw (-9.3,0) node[G-node,label=center:$0$,label=below:$a'_3$] (a'_3) {};
\draw (-12.3,0) node[G-node,label=center:$1$,label=below:$a'_4$] (a'_4) {};




\draw (3,0) node[G-node,label=center:$0$,label=below:$b'_1$] (b'_1) {};
\draw (6,0) node[G-node,label=center:$1$,label=below:$b'_2$] (b'_2) {};
\draw (9.3,0) node[G-node,label=center:$0$,label=below:$b'_3$] (b'_3) {};
\draw (12.3,0) node[G-node,label=center:$1$,label=below:$b'_4$] (b'_4) {};
\draw (15.6,0) node[G-node,label=center:$1$,label=below:$b'_5$] (b'_5) {};


\draw[b9] (r)  to node [below,label=right:] {} (a'_1) ;
\draw[b9] (a'_1)  to node [below,label=right:] {} (a'_2) ;
\draw[b9] (a'_2)  to node [below,label=right:] {} (a'_3) ;
\draw[b9] (a'_3)  to node [below,label=below:] {} (a'_4) ;

\draw[b9] (r)  to node [below,label=right:] {} (c'_1) ;
\draw[b9] (c'_1)  to node [below,label=right:] {} (c'_2) ;
\draw[b9] (c'_8)  to node [below,label=below:] {} (c'_9) ;

\draw[b9] (r)  to node [below,label=right:] {} (b'_1) ;
\draw[b9] (b'_1)  to node [below,label=right:] {} (b'_2) ;
\draw[b9] (b'_2)  to node [below,label=right:] {} (b'_3) ;
\draw[b9] (b'_3)  to node [below,label=below:] {} (b'_4) ;
\draw[b9] (b'_4)  to node [below,label=below:] {} (b'_5) ;

%\draw[b9] (b_2)  to node [label=right:$q_{B1}$] {} (h_1) ;
%\draw (3, 8) node[W-node,label=center:First Scenario] (s1) {};

%\draw (9,5) node[B-node,label=center:$A$,label=below:$\pi_A$\text{$=$}$0.0938$] (bb_1) {};
%\draw (13,5) node[B-node,label=center:$B$,label=below:$\pi_B$\text{$=$}$0.0938$] (bb_2) {};
%\draw (9,0) node[R-node,label=center:$1$, label=below:$p_1$\text{$=$}$\frac{1}{2}$] (hh_1) {};
%\draw (13,0) node[R-node,label=center:$2$, label=below:$p_2$\text{$=$}$\frac{1}{2}$] (hh_2) {};

%\draw[b9] (bb_1) to node [label=left:$q_{A1}$] {} (hh_1) ;
%\draw[b9] (bb_1) -- (hh_2) ;
%\draw[b9] (bb_2) -- (hh_1) ;
%\draw[b9] (bb_2) to node [label=right:$q_{B2}$] {} (hh_2) ;
%\draw (11, 8) node[W-node,label=center:Second Scenario] (s2) {};

%\draw (9.8, 3) node[W-node,label=center:$q_{A2}$] (lab2) {};
%\draw (12.2, 3) node[W-node,label=center:$q_{B1}$] (lab3) {};

%\draw (17,5) node[B-node,label=center:$A$,label=below:$\pi_A$\text{$=$}$0.124$] (bbb_1) {};
%\draw (21,5) node[B-node,label=center:$B$,label=below:$\pi_B$\text{$=$}$0.064$] (bbb_2) {};
%\draw (17,0) node[R-node,label=center:$1$, label=below:$p_1$\text{$=$}$0.64$] (hhh_1) {};
%\draw (21,0) node[R-node,label=center:$2$, label=below:$p_2$\text{$=$}$0.48$] (hhh_2) {};

%\draw[b9] (bbb_1)  to node [label=left:$q_{A1}$] {} (hhh_1) ;
%\draw[b9] (bbb_1)  to node [label=left:$q_{A2}$] {} (hhh_2) ;
%\draw[b9] (bbb_2)  to node [label=right:$q_{B2}$] {} (hhh_2) ;
%\draw (19, 8) node[W-node,label=center:Third Scenario] (s3) {};
\end{tikzpicture}
\end{center}
\caption{The above tree corresponds to vectors $a = \langle 0,1,3,4 \rangle$ and $b = \langle 0,2,4,5\rangle$.}
\label{fig:treesparsity}
\end{figure}

==> windows.tex <==
\begin{figure}[h!]

\begin{center}
\begin{tikzpicture}[scale=0.96, transform shape]

%\draw (0,0) -- (15.4,0) -- (15.4,0.5) -- (0,0.5) -- (0,0);
%\node[text width=3cm] at (9,0.2) 
%{$a$};

%\node[text width=3cm, rotate = 90] at (-0.5,2.6) 
%{    \Huge$\overbrace{\hspace{3.9cm}}$   };
%\node[text width=3cm, rotate = 90] at (-1.3,3.2) 
%{  $\log n +1$ rounds  };

%\node[text width=3cm] at (3.9,5.2) 
%{    \huge$\overbrace{\hspace{3.0cm}}$   };



\node[text width=3cm, rotate = 90] at (7.72,4.1) 
{  \huge  $\ldots$   };

\draw (-0.1,1.1) -- (15.5,1.1) -- (15.5,1.8) -- (-0.1,1.8) -- (-0.1,1.1);
\draw[dashed] (0,1.2) -- (0.4,1.2) -- (0.4,1.7) -- (0,1.7) -- (0,1.2);
\draw[dashed] (0.5,1.2) -- (0.9,1.2) -- (0.9,1.7) -- (0.5,1.7) -- (0.5,1.2);
\draw[dashed] (1,1.2) -- (1.4,1.2) -- (1.4,1.7) -- (1,1.7) -- (1,1.2);
\draw[dashed] (1.5,1.2) -- (1.9,1.2) -- (1.9,1.7) -- (1.5,1.7) -- (1.5,1.2);
\draw[dashed] (2,1.2) -- (2.4,1.2) -- (2.4,1.7) -- (2,1.7) -- (2,1.2);
\draw[dashed] (2.5,1.2) -- (2.9,1.2) -- (2.9,1.7) -- (2.5,1.7) -- (2.5,1.2);
\draw[dashed] (3,1.2) -- (3.4,1.2) -- (3.4,1.7) -- (3,1.7) -- (3,1.2);
\draw[dashed] (3.5,1.2) -- (3.9,1.2) -- (3.9,1.7) -- (3.5,1.7) -- (3.5,1.2);
\draw[dashed] (4,1.2) -- (4.4,1.2) -- (4.4,1.7) -- (4,1.7) -- (4,1.2);
\draw[dashed] (4.5,1.2) -- (4.9,1.2) -- (4.9,1.7) -- (4.5,1.7) -- (4.5,1.2);
\draw[dashed] (5,1.2) -- (5.4,1.2) -- (5.4,1.7) -- (5,1.7) -- (5,1.2);
\draw[dashed] (5.5,1.2) -- (5.9,1.2) -- (5.9,1.7) -- (5.5,1.7) -- (5.5,1.2);
\draw[dashed] (6,1.2) -- (6.4,1.2) -- (6.4,1.7) -- (6,1.7) -- (6,1.2);
\draw[dashed] (6.5,1.2) -- (6.9,1.2) -- (6.9,1.7) -- (6.5,1.7) -- (6.5,1.2);



\draw[dashed] (8.5,1.2) -- (8.9,1.2) -- (8.9,1.7) -- (8.5,1.7) -- (8.5,1.2);
\draw[dashed] (9,1.2) -- (9.4,1.2) -- (9.4,1.7) -- (9,1.7) -- (9,1.2);
\draw[dashed] (9.5,1.2) -- (9.9,1.2) -- (9.9,1.7) -- (9.5,1.7) -- (9.5,1.2);
\draw[dashed] (10,1.2) -- (10.4,1.2) -- (10.4,1.7) -- (10,1.7) -- (10,1.2);
\draw[dashed] (10.5,1.2) -- (10.9,1.2) -- (10.9,1.7) -- (10.5,1.7) -- (10.5,1.2);
\draw[dashed] (11,1.2) -- (11.4,1.2) -- (11.4,1.7) -- (11,1.7) -- (11,1.2);
\draw[dashed] (11.5,1.2) -- (11.9,1.2) -- (11.9,1.7) -- (11.5,1.7) -- (11.5,1.2);
\draw[dashed] (12,1.2) -- (12.4,1.2) -- (12.4,1.7) -- (12,1.7) -- (12,1.2);
\draw[dashed] (12.5,1.2) -- (12.9,1.2) -- (12.9,1.7) -- (12.5,1.7) -- (12.5,1.2);
\draw[dashed] (13,1.2) -- (13.4,1.2) -- (13.4,1.7) -- (13,1.7) -- (13,1.2);
\draw[dashed] (13.5,1.2) -- (13.9,1.2) -- (13.9,1.7) -- (13.5,1.7) -- (13.5,1.2);
\draw[dashed] (14,1.2) -- (14.4,1.2) -- (14.4,1.7) -- (14,1.7) -- (14,1.2);
\draw[dashed] (14.5,1.2) -- (14.9,1.2) -- (14.9,1.7) -- (14.5,1.7) -- (14.5,1.2);
\draw[dashed] (15,1.2) -- (15.4,1.2) -- (15.4,1.7) -- (15,1.7) -- (15,1.2);
%\draw[dashed] (6.2,1.2) -- (9.2,1.2) -- (9.2,1.7) -- (6.2,1.7) -- (6.2,1.2);
\node[text width=3cm] at (8.8,1.4) 
{   \huge $\ldots$   };

\node[text width=3cm] at (17.1,1.4) 
{   round $\log n +1$  };

%\draw[dashed] (9.3,1.2) -- (12.3,1.2) -- (12.3,1.7) -- (9.3,1.7) -- (9.3,1.2);
%\draw[dashed] (12.4,1.2) -- (15.4,1.2) -- (15.4,1.7) -- (12.4,1.7) -- (12.4,1.2);

%\draw[dashed] (0.6,2) -- (3.6,2) -- (3.6,2.5) -- (0.6,2.5) -- (0.6,2);
%\draw[dashed] (3.7,2) -- (6.7,2) -- (6.7,2.5) -- (3.7,2.5) -- (3.7,2);
%\draw[dashed] (6.8,2) -- (9.8,2) -- (9.8,2.5) -- (6.8,2.5) -- (6.8,2);

\draw (-0.1,1.9) -- (15.5,1.9) -- (15.5,2.6) -- (-0.1,2.6) -- (-0.1,1.9);
\draw[dashed] (0,2) -- (0.9,2) -- (0.9,2.5) -- (0,2.5) -- (0,2);
\draw[dashed] (1,2) -- (1.9,2) -- (1.9,2.5) -- (1,2.5) -- (1,2);
\draw[dashed] (2,2) -- (2.9,2) -- (2.9,2.5) -- (2,2.5) -- (2,2);
\draw[dashed] (3,2) -- (3.9,2) -- (3.9,2.5) -- (3,2.5) -- (3,2);
\draw[dashed] (4,2) -- (4.9,2) -- (4.9,2.5) -- (4,2.5) -- (4,2);
\draw[dashed] (5,2) -- (5.9,2) -- (5.9,2.5) -- (5,2.5) -- (5,2);
\draw[dashed] (6,2) -- (6.9,2) -- (6.9,2.5) -- (6,2.5) -- (6,2);


\draw[dashed] (8.5,2) -- (9.4,2) -- (9.4,2.5) -- (8.5,2.5) -- (8.5,2);
\draw[dashed] (9.5,2) -- (10.4,2) -- (10.4,2.5) -- (9.5,2.5) -- (9.5,2);
\draw[dashed] (10.5,2) -- (11.4,2) -- (11.4,2.5) -- (10.5,2.5) -- (10.5,2);
\draw[dashed] (11.5,2) -- (12.4,2) -- (12.4,2.5) -- (11.5,2.5) -- (11.5,2);
\draw[dashed] (12.5,2) -- (13.4,2) -- (13.4,2.5) -- (12.5,2.5) -- (12.5,2);
\draw[dashed] (13.5,2) -- (14.4,2) -- (14.4,2.5) -- (13.5,2.5) -- (13.5,2);
\draw[dashed] (14.5,2) -- (15.4,2) -- (15.4,2.5) -- (14.5,2.5) -- (14.5,2);

\node[text width=3cm] at (8.8,2.2) 
{   \huge $\ldots$   };
%\draw[dashed] (9.9,2) -- (12.9,2) -- (12.9,2.5) -- (9.9,2.5) -- (9.9,2);
\node[text width=3cm] at (17.1,2.2) 
{   round $\log n$  };


%\draw[dashed] (1.2,2.8) -- (4.2,2.8) -- (4.2,3.3) -- (1.2,3.3) -- (1.2,2.8);
%\draw[dashed] (4.3,2.8) -- (7.3,2.8) -- (7.3,3.3) -- (4.3,3.3) -- (4.3,2.8);
%\draw[dashed] (7.4,2.8) -- (10.4,2.8) -- (10.4,3.3) -- (7.4,3.3) -- (7.4,2.8);
%\node[text width=3cm] at (10.0,3.0) 
%{   \huge $\ldots$   };
%\draw[dashed] (10.5,2.8) -- (13.5,2.8) -- (13.5,3.3) -- (10.5,3.3) -- (10.5,2.8);

\draw (-0.1,3.5) -- (15.5,3.5) -- (15.5,4.2) -- (-0.1,4.2) -- (-0.1,3.5);
\draw[dashed] (0,3.6) -- (7.6,3.6) -- (7.6,4.1) -- (0,4.1) -- (0,3.6);
%\draw[dashed] (1.8,3.6) -- (4.8,3.6) -- (4.8,4.1) -- (1.8,4.1) -- (1.8,3.6);
%\draw[dashed] (4.9,3.6) -- (7.9,3.6) -- (7.9,4.1) -- (4.9,4.1) -- (4.9,3.6);
%\draw[dashed] (8.0,3.6) -- (11.0,3.6) -- (11.0,4.1) -- (8.0,4.1) -- (8.0,3.6);
\draw[dashed] (7.8,3.6) -- (15.4,3.6) -- (15.4,4.1) -- (7.8,4.1) -- (7.8,3.6);
%\draw[dashed] (11.1,3.6) -- (14.1,3.6) -- (14.1,4.1) -- (11.1,4.1) -- (11.1,3.6);

\node[text width=3cm] at (17.1,3.8) 
{   round $2$  };

\draw (-0.1,4.3) -- (15.5,4.3) -- (15.5,5) -- (-0.1,5) -- (-0.1,4.3);
\draw[dashed] (0,4.4) -- (15.4,4.4) -- (15.4,4.9) -- (0,4.9) -- (0,4.4);
\node[text width=3cm] at (17.1,4.6) 
{   round $1$  };

\node[text width=3cm] at (1.42,5.3) 
{   $1$   };
\node[text width=3cm] at (16.62,5.3) 
{   $n$   };
%\draw[dashed] (2.4,4.4) -- (5.4,4.4) -- (5.4,4.9) -- (2.4,4.9) -- (2.4,4.4);
%\draw[dashed] (5.5,4.4) -- (8.5,4.4) -- (8.5,4.9) -- (5.5,4.9) -- (5.5,4.4);
%\draw[dashed] (8.6,4.4) -- (11.6,4.4) -- (11.6,4.9) -- (8.6,4.9) -- (8.6,4.4);
%\node[text width=3cm] at (11.2,4.6) 
%{   \huge $\ldots$   };
%\draw[dashed] (11.7,4.4) -- (14.7,4.4) -- (14.7,4.9) -- (11.7,4.9) -- (11.7,4.4);




%\node [draw,rounded corners,minimum height=5cm,minimum width=4cm] (node1) {};
%\node [anchor=north west,minimum width=10cm] at (-3.6,1) {\fbox{\hspace{1cm}$w_1$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (-0.9,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (1.8,1) {\fbox{\hspace{1cm}$\ldots$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (4.5,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (7.2,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (0,0) {\fbox{\hspace{6.4cm}$s_1$\hspace{6.4cm}}};
% {\fbox{\hspace{6.4cm}$s_1$\hspace{6.4cm}}};

%\node [anchor=south west] at (node1.north west) {\fbox{Case: anchor is SW}};
%\node [anchor=south east] at (node1.north west) {\fbox{Case: anchor is SE}};
%\node [anchor=north east] at (node1.north west) {\fbox{Case: anchor is NE}};
%\foreach \myanchor in {north west}
%{ 
%	\node[fill,circle,inner sep=1pt,outer sep=1ex,anchor=\myanchor] at (node1.north west){};
%}
\end{tikzpicture}
\end{center}
\caption{In every round $s+1$, $b$ is split into $2^s$ intervals of size $2^{\log n - s}$.}\label{figs:bs}
\end{figure}
